Maximum likelihood estimation for a stochastic SEIR system for COVID-19

The parameter estimation of epidemic data-driven models is a crucial task. In some cases, we can formulate a better model by describing uncertainty with appropriate noise terms. However, because of the limited extent and partial information, (in general) this kind of model leads to intractable likelihoods. Here, we illustrate how a stochastic extension of the SEIR model improves the uncertainty quantification of an overestimated MCMC scheme based on its deterministic model to count reported-confirmed COVID-19 cases in Mexico City. Using a particular mechanism to manage missing data, we developed MLE for some parameters of the stochastic model, which improves the description of variance of the actual data.

==> bibliography.tex <==

\bibliography{References}
\bibstyle{rss}



==> estimation.tex <==
By applying Lamperti's transformation  in the equation for $S$ we have that 

\begin{align}
-\frac{1}{\sigma}d\big(\log (1-S_t) \big)&= \Big[ \mu \frac{1-S}{\sigma(1-S)} -\frac{\beta  S I_s}{\sigma (1-S)} + \frac{\gamma  R}{\sigma (1-S)} + \tfrac{1}{2} \sigma \Big] dt + dW(t)\nonumber \\
&=\Big[  \frac{\mu}{\sigma } -\frac{\beta  S I_s}{\sigma (1-S)} + \frac{\gamma  R}{\sigma (1-S)} + \tfrac{1}{2} \sigma \Big] dt + dW(t). \label{dlogS}
\end{align}


Again, by  Lamperti's transformation in the equation for $E$ we have that 
\begin{align}
-\frac{1}{\sigma} d(\log (E_t))&= \Big[ -\frac{\beta  S I_s }{\sigma E} +\frac{\kappa p E}{\sigma E} +\frac{\mu E}{\sigma E}  +  \frac{1}{2} \sigma\Big] dt + dW(t)\nonumber \\ 
& = \Big[ -\frac{\beta  S I_s }{\sigma E} + \frac{\kappa p }{\sigma }  + \frac{\mu }{\sigma }  +  \frac{1}{2} \sigma\Big] dt + dW(t)\label{dlogE}
\end{align}
In very similar manner we obtain the transformation, via Lamperti, for  $I_a,I_s,R$:
 \begin{align}
-\frac{1}{\sigma} d(\log (I_a))&= \Big[ -\frac{\kappa p E}{\sigma I_a} + \frac{(\alpha_a + \mu )I_a}{\sigma I_a}  +  \frac{1}{2} \sigma\Big] dt + dW(t)\nonumber \\ 
& = \Big[ -\frac{\kappa p E}{\sigma I_a} +\frac{(\alpha_a + \mu )}{\sigma }  +  \frac{1}{2} \sigma\Big] dt + dW(t) \label{dlogIa}
\end{align}

 \begin{align}
-\frac{1}{\sigma} d(\log (I_s))&= \Big[ -\frac{\kappa (1-p) E}{\sigma I_s} + \frac{(\alpha_s + \mu )I_s}{\sigma I_s}  +  \frac{1}{2} \sigma\Big] dt + dW(t)\nonumber \\ 
& = \Big[ -\frac{\kappa (1-p) E}{\sigma I_s} + \frac{(\alpha_s + \mu )}{\sigma } +  \frac{1}{2} \sigma\Big] dt + dW(t) \label{dlogIs}
\end{align}
 \begin{align}
-\frac{1}{\sigma} d(\log (R))&= \Big[ - \frac{\alpha_a I_a + \alpha_s I_s}{\sigma R} + \frac{\mu + \gamma}{\sigma } +  \frac{1}{2} \sigma\Big] dt + dW(t)\label{dlogR}
\end{align}

   
Then, we can write these SDEs as a five dimensions system of SDEs:
\begin{equation}\label{dlog-SE}
-\frac{1}{\sigma} d \mathbf{X}_{\beta,p} = F(\mathbf{X}_{\beta,p}) dt + d\mathbf{W}
\end{equation}  
where, 
\begin{equation*}
 \mathbf{X}_{\beta,p} := \begin{pmatrix}
 \log (1-S)\\ \log (E) \\
 \log (I_a)\\  \log (I_s) \\  \log (R)
\end{pmatrix},\quad F(\mathbf{X}_{\beta,p}):=  \begin{pmatrix}
 \frac{\mu}{\sigma } -\frac{\beta  S I_s}{\sigma (1-S)} + \frac{\gamma  R}{\sigma (1-S)} + \tfrac{1}{2} \sigma  \\ 
-\frac{\beta  S I_s }{\sigma E} + \frac{\kappa p }{\sigma }  + \frac{\mu }{\sigma }  +  \frac{1}{2} \sigma \\
-\frac{\kappa p E}{\sigma I_a} +\frac{(\alpha_a + \mu )}{\sigma }  +  \frac{1}{2} \sigma \\
-\frac{\kappa (1-p) E}{\sigma I_s} + \frac{(\alpha_s + \mu )}{\sigma }  +  \frac{1}{2} \sigma \\
- \frac{\alpha_a I_a + \alpha_s I_s}{\sigma R} + \frac{\mu + \gamma}{\sigma } + \frac{1}{2} \sigma
\end{pmatrix},\quad  d\mathbf{W}:=\begin{pmatrix}
dW(t)\\ dW(t) \\ dW(t)\\ dW(t) \\ dW(t)
\end{pmatrix}
\end{equation*}   
    
    
    
    
%    \section{Data and methods}
\section{MLE for the $\beta$}

We will apply the version of the  Girsanov formula presented in \cite[see Theorem 7.4 therein]{saso19} for the system \eqref{dlog-SE}. We will assume that the true value of the parameters $\beta_0, p_0$ are unknown. Denote by $\Pb_{\beta,p}$ the law for the solution of \eqref{dlog-SE}. It is known that the measures $\Pb_\beta$ are equivalent for different values of $\beta$ (see for instance \cite{iacus}, \cite{Bishwal2008}, \cite{saso19}. Then, by Theorem 7.4 in \cite{saso19},  we have that the likelihood ratio, or Radon-Nikodyn derivative has the form 
\begin{align}
\frac{d\Pb_\beta}{d\Pb_{\beta_0}} &= \exp\Bigg[ \int_0^T [ F(\mathbf{X}_{\beta,p}(t))  - F(\mathbf{X}_{\beta_0,p_0}(t)) ]^{T} Q^{-1} d\mathbf{W}(t) \nonumber\\
&\qquad \quad -\frac{1}{2} \int_0^T  [ F(\mathbf{X}_{\beta,p}(t))  - F(\mathbf{X}_{\beta_0,p_0}(t)) ]^{T}Q^{-1}  [ F(\mathbf{X}_{\beta,p}(t))  - F(\mathbf{X}_{\beta_0,p_0}(t)) ] d(t)\Bigg] \label{Likelihood}
\end{align}
where $Q$, in our case, is the 5-identity matrix and 

\begin{align*}
 [ F(\mathbf{X}_{\beta,p}(t))  - F(\mathbf{X}_{\beta_0,p_0}(t)) ]  &= \begin{pmatrix}
 -(\beta-\beta_0) \frac{S(t) I_s(t)}{\sigma (1-S(t))} \\ 
-(\beta-\beta_0) \frac{S(t) I_s(t)}{\sigma E(t)} + (p-p_0)\frac{\kappa}{\sigma}  \\
-(p-p_0)\frac{\kappa E(t)}{\sigma I_a(t)}   \\
(p-p_0)\frac{\kappa E(t)}{\sigma I_s(t)}   \\
0
\end{pmatrix},
\end{align*}
  
thus, 
\begin{align*}
 [ F(\mathbf{X}_{\beta,p}(t)) & - F(\mathbf{X}_{\beta_0,p_0}(t)) ]^{T} Q^{-1} d\mathbf{W}(t)  \\
 &= -(\beta-\beta_0) \frac{S(t) I_s(t)}{\sigma (1-S(t))} dW(t) -(\beta-\beta_0) \frac{S(t) I_s(t)}{\sigma E(t)} dW(t)+ (p-p_0)\frac{\kappa}{\sigma}  dW(t)  \\
 &\quad -(p-p_0)\frac{\kappa E(t)}{\sigma I_a(t)} dW(t) +
(p-p_0)\frac{\kappa E(t)}{\sigma I_s(t)} dW(t) ,
\end{align*}
and 
\begin{align*}
 [ F(\mathbf{X}_{\beta,p}(t)) & - F(\mathbf{X}_{\beta_0,p_0}(t)) ]^{T}Q^{-1}   [ F(\mathbf{X}_{\beta,p}(t))  - F(\mathbf{X}_{\beta_0,p_0}(t)) ]  \\
 &=\Big[ -(\beta-\beta_0) \frac{S(t) I_s(t)}{\sigma (1-S(t))} \Big]^2 + \Big[-(\beta-\beta_0) \frac{S(t) I_s(t)}{\sigma E(t)} +   (p-p_0)\frac{\kappa}{\sigma}\Big]^2 \\
 &\quad + \Big[ -(p-p_0) \frac{\kappa E(t)}{\sigma I_a(t)} \Big]^2 +
\Big[ (p-p_0)\frac{\kappa E(t)}{\sigma I_s(t)}\Big]^2.
\end{align*}
   
    By maximizing the log likelihood with respect to $\beta$ we have that 
 \begin{align*}
0 &=  \int_0^T \Big[ - \frac{S(t) I_s(t)}{\sigma (1-S(t))} -  \frac{S(t) I_s(t)}{\sigma E(t)} \Big]  dW(t)  \\
 &\quad -\frac{1}{2}  \int_0^T \left( 2 (\beta-\beta_0)   \Big[ \frac{S(t) I_s(t)}{\sigma (1-S(t))} \Big]^2  +  2 (\beta-\beta_0)   \Big[ \frac{S(t) I_s(t)}{\sigma E(t)} \Big]^2 
 - 2 \frac{\kappa}{\sigma} (p-p_0) \frac{S(t) I_s(t)}{\sigma E(t)}\right) dt.
\end{align*}
  
then, 
\begin{align*}
(\beta-\beta_0) \int_0^T \left(  \Big[ \frac{S(t) I_s(t)}{ (1-S(t))} \Big]^2  +   \Big[ \frac{S(t) I_s(t)}{ E(t)} \Big]^2 \right) dt &=  {\color{blue} +}  (p-p_0)\, \kappa   \int_0^T  \frac{S(t) I_s(t)}{ E(t)} dt \\
& - {\color{blue} \sigma } \int_0^T \Big[ \frac{S(t) I_s(t)}{ (1-S(t))} +  \frac{S(t) I_s(t)}{ E(t)} \Big]  dW(t)
\end{align*}
   
   which implies that 

\begin{equation}\label{MLE-beta-beta0}
\hat{\beta}_{ML} - \beta_0 = \frac{1}{J_1(T)}\left[  (p-p_0) \, \kappa   \int_0^T   \frac{S(t) I_s(t)}{ E(t)} dt \\
- \sigma  \int_0^T \Big[ \frac{S(t) I_s(t)}{ (1-S(t))} +  \frac{S(t) I_s(t)}{ E(t)} \Big]  dW(t)\right]
\end{equation}
   with 
$$
J_1(T):= \int_0^T \left(  \Big[ \frac{S(t) I_s(t)}{ (1-S(t))} \Big]^2  +   \Big[ \frac{S(t) I_s(t)}{ E(t)} \Big]^2 \right) dt.
$$   

    
    At other hand,   by maximizing the log likelihood with respect to $p$ we have that 
    
  \begin{align*}
0 &=  \int_0^T \Big[  -\frac{\kappa E(t)}{\sigma I_a(t)} dW(t) +
\frac{\kappa E(t)}{\sigma I_s(t)} dW(t) \Big] - \frac{1}{2} \int_0^T 2 \Big[-(\beta-\beta_0) \frac{S(t)I_s(t)}{\sigma E(t)} + \frac{\kappa}{\sigma} (p-p_0) \Big] \frac{\kappa}{\sigma} d(t)\\
& + \frac{\kappa}{\sigma} W(T) - \frac{1}{2} \int_0^T 2 (p-p_0)\Big[ \frac{\kappa^2 E^2(t)}{\sigma^2 I_s^2(t)} +  \frac{\kappa^2 E^2(t)}{\sigma^2 I_a^2(t)} \Big] dt,
   \end{align*} 
then,     
    \begin{align*}
(p-p_0)\left( \kappa^2 T + \int_0^T  \Big[ \frac{\kappa^2 E^2(t)}{ I_s^2(t)} +  \frac{\kappa^2 E^2(t)}{ I_a^2(t)} \Big] dt \right) &= \sigma \int_0^T \Big[  -\frac{\kappa E(t)}{ I_a(t)} +
\frac{\kappa E(t)}{ I_s(t)} \Big] dW(t) \\
& + \sigma \kappa W(T)  + (\beta-\beta_0) \kappa \int_0^T \frac{S(t)I_s(t)}{ E(t)} dt.
  \end{align*}   
    
This implies that     
     \begin{align}\label{MLE_p}
\hat{p}_{ML}-p_0 &=  \frac{\kappa \sigma}{J_2(T) } W(T) + \frac{\kappa}{J_2(T)}(\beta-\beta_0) \int_0^T \frac{S(t)I_s(t)}{ E(t)} dt +  \frac{\sigma }{J_2(T)} \int_0^T \Big[  -\frac{\kappa E(t)}{ I_a(t)} +
\frac{\kappa E(t)}{ I_s(t)} \Big] dW(t),
  \end{align}
with 
$$
J_2(T):= \kappa^2 T + \int_0^T  \Big[ \frac{\kappa^2 E^2(t)}{ I_s^2(t)} +  \frac{\kappa^2 E^2(t)}{ I_a^2(t)}\Big] dt.
$$
  
 We can rewrite the equations  \eqref{MLE-beta-beta0} and \eqref{MLE_p} as
 
\begin{equation*}
 \begin{pmatrix}
J_1(T)  &   -\kappa \int_0^T \frac{S(t)I_s(t)}{ E(t)} dt  \\ 
-\kappa \int_0^T \frac{S(t)I_s(t)}{E(t)} dt   & J_2(T)
\end{pmatrix} 
\begin{pmatrix}
\hat \beta_{ML}-\beta_0
\\
\hat p_{ML}-p_0
\end{pmatrix} = - \sigma
  \begin{pmatrix}
  \int_0^T \Big[ \frac{S(t) I_s(t)}{ (1-S(t))} +  \frac{S(t) I_s(t)}{ E(t)} \Big]  dW(t)
  \\ 
- \kappa W(T)  + \int_0^T \Big[  \frac{\kappa E(t)}{ I_a(t)} -
\frac{\kappa E(t)}{ I_s(t)} \Big] dW(t). 
\end{pmatrix}
\end{equation*}   

Thus, 
  
\begin{equation}
\begin{pmatrix}
\hat \beta_{ML} -\beta_0
\\
\hat p_{ML} -p_0
\end{pmatrix} = - \sigma\begin{pmatrix}
J_1(T)  &   -\kappa \int_0^T \frac{S(t)I_s(t)}{ E(t)} dt  \\ 
-\kappa \int_0^T \frac{S(t)I_s(t)}{E(t)} dt   & J_2(T)
\end{pmatrix}^{-1} 
  \begin{pmatrix}
  \int_0^T \Big[ \frac{S(t) I_s(t)}{ (1-S(t))} +  \frac{S(t) I_s(t)}{ E(t)} \Big]  dW(t)
  \\ 
 - \kappa W(T)  + \int_0^T \Big[  \frac{\kappa E(t)}{\sigma I_a(t)} -
\frac{\kappa E(t)}{\sigma I_s(t)} \Big] dW(t). 
\end{pmatrix}
\end{equation}      
     
We have the following result.
  \begin{theorem}
The estimators $(\hat{\beta}_{ML},\hat{p}_{ML})$ are jointly strongly consistent, i.e.
\begin{equation}\label{consistency}
\lim_{T \rightarrow \infty} \begin{pmatrix}
\hat \beta_{ML} 
\\
\hat p_{ML}
\end{pmatrix}= \begin{pmatrix}
\beta_0
\\
p_0
\end{pmatrix}, \qquad \mbox{with probability one}
\end{equation}
and asymtotically normal, i.e.
\begin{equation}\label{normality}
\lim_{T \rightarrow \infty} C_T \begin{pmatrix}
\hat \beta_{ML} -\beta_0
\\
\hat p_{ML} -p_0
\end{pmatrix}  = \begin{pmatrix} 
\mathcal{N}(0,1) \\ \mathcal{N}(0,1) 
\end{pmatrix}, \qquad \mbox{with probability one}
\end{equation}
where 
$$
C_T:=\sigma \sqrt{Var\left( \det \begin{pmatrix}
J_1(T)  &   -\kappa \int_0^T \frac{S(t)I_s(t)}{ E(t)} dt  \\ 
-\kappa \int_0^T \frac{S(t)I_s(t)}{E(t)} dt   & J_2(T)
\end{pmatrix}^{-1}  \right)}
$$
\end{theorem}
\begin{proof} 
    
    
 \end{proof}
   
  \begin{remark}
   
   It is possible to prove that 
   
\begin{align}\label{beta_hat}
J_1(T)\, \hat{\beta}_{ML}  &=   {\color{red}  \hat{p}_{ML} }\kappa  \int_0^T  \frac{S(t)  I_s(t)}{E(t)}dt + \int_0^T  \frac{S(t)  I_s(t)}{ [1-S(t)]} d \big(\ln [1-S(t)]\big)\nonumber\\
&\quad + \int_0^T  \frac{S(t)  I_s(t)}{ E(t)} d \big(\ln E(t) \big) +\frac{1}{2}\sigma^2  \int_0^T S(t)I_s(t) \Big[\frac{1}{E(t)} + \frac{1}{1-S(t)}  \Big] dt \nonumber\\
&\quad + \mu \int_0^T  S(t)  I_s(t) \Big[  \frac{1}{E(t)} + \frac{1}{1-S(t)} \Big] dt + \gamma \int_0^T  \frac{R(t) S(t)  I_s(t)}{ \big(1-S(t) \big)^2} dt, 
\end{align}  
and
\begin{align}\label{p_hat}
J_2(T)\, \hat{p}_{ML}  &=   {\color{red}  \hat{\beta}_{ML} } \kappa \int_0^T \frac{S(t) I_S(t)}{E(t)} dt   +  \kappa^2 \int_0^T \frac{E^2(t) }{I_S^2(t)} dt - \kappa \int_0^T \frac{E(t) }{I_S(t)} d\big(\ln (I_S(t)) \big)   \nonumber \\
 &\quad -  \kappa (\alpha_S+\mu) \int_0^T \frac{E(t) }{I_S(t)} dt - \frac{1}{2}\kappa\sigma^2 \int_0^T \frac{E(t) }{I_S(t)} dt + \kappa \int_0^T \frac{E(t) }{I_a(t)} d\big(\ln (I_a(t)) \big) \nonumber \\
 &\quad  + \kappa (\alpha_a+\mu) \int_0^T \frac{E(t) }{I_a(t)} dt + \frac{1}{2}\kappa \sigma^2 \int_0^T \frac{E(t) }{I_a(t)} dt - \kappa \ln \Big(\frac{E(t)}{E(0)}\Big) - \kappa \Big( \mu + \frac{1}{2}\sigma^2 \Big) T,
\end{align}  
which can be writen as the system:


\begin{equation}\label{matrix-beta-p}
 \begin{pmatrix}
J_1(T)  &   -\kappa \int_0^T \frac{S(t)I_s(t)}{ E(t)} dt  \\ 
-\kappa \int_0^T \frac{S(t)I_s(t)}{E(t)} dt   & J_2(T)
\end{pmatrix} 
\begin{pmatrix}
\hat \beta_{ML}
\\
\hat p_{ML}
\end{pmatrix} = 
  \begin{pmatrix}
  R_1(T)
  \\ 
 R_2(T). 
\end{pmatrix}
\end{equation}   
with $R_1$ and $R_2$ being
\begin{align*}
R_1(T)& = \int_0^T  \frac{S(t)  I_s(t)}{ [1-S(t)]} d \big(\ln [1-S(t)]\big)\nonumber\\
&\quad + \int_0^T  \frac{S(t)  I_s(t)}{ E(t)} d \big(\ln E(t) \big) +\frac{1}{2}\sigma^2  \int_0^T S(t)I_s(t) \Big[\frac{1}{E(t)} + \frac{1}{1-S(t)}  \Big] dt \nonumber\\
&\quad + \mu \int_0^T  S(t)  I_s(t) \Big[  \frac{1}{E(t)} + \frac{1}{1-S(t)} \Big] dt + \gamma \int_0^T  \frac{R(t) S(t)  I_s(t)}{ \big(1-S(t) \big)^2} dt \\
R_2(T)& =  \kappa^2 \int_0^T \frac{E^2(t) }{I_S^2(t)} dt - \kappa \int_0^T \frac{E(t) }{I_S(t)} d\big(\ln (I_S(t)) \big)   \nonumber \\
 &\quad -  \kappa (\alpha_S+\mu) \int_0^T \frac{E(t) }{I_S(t)} dt - \frac{1}{2}\kappa\sigma^2 \int_0^T \frac{E(t) }{I_S(t)} dt + \kappa \int_0^T \frac{E(t) }{I_a(t)} d\big(\ln (I_a(t)) \big) \nonumber \\
 &\quad  + \kappa (\alpha_a+\mu) \int_0^T \frac{E(t) }{I_a(t)} dt + \frac{1}{2}\kappa \sigma^2 \int_0^T \frac{E(t) }{I_a(t)} dt - \kappa \ln \Big(\frac{E(t)}{E(0)}\Big) - \kappa \Big( \mu + \frac{1}{2}\sigma^2 \Big) T .
\end{align*}
 Then, from \eqref{matrix-beta-p}
 
 \begin{equation}\label{beta-p}
 \begin{pmatrix}
\hat \beta_{ML}
\\
\hat p_{ML}
\end{pmatrix} = \begin{pmatrix}
J_1(T)  &   -\kappa \int_0^T \frac{S(t)I_s(t)}{ E(t)} dt  \\ 
-\kappa \int_0^T \frac{S(t)I_s(t)}{E(t)} dt   & J_2(T)
\end{pmatrix}^{-1} 
  \begin{pmatrix}
  R_1(T)
  \\ 
 R_2(T). 
\end{pmatrix}
\end{equation}
\end{remark}


==> frontmatter.tex <==
    \author[1\authfn{1}]{Fernando Baltazar-Larios}
    \author[2\authfn{2}]{Francisco Delgado-Vences} 
    \author[3\authfn{3}]{Saul Diaz-Infante*}
    \contrib[\authfn{1}]{Equally contributing authors. Authors are listed alphabetically.}
    %
    \affil[1]{%
    Departamento de Matem\'aticas, 
        Facultad de Ciencias, %
        UNAM, %
        Ciudad de M\'exico, %
        M\'exico%
    }
    \affil[2]{%
   CONACYT - Instituto de Mat\'ematicas, Unidad Oaxaca\, %
        UNAM,\, %
        Oaxaca de Juarez,\,%
        M\'exico%
    }
    \corraddress{%
        Departamento de Matem\'aticas, %
        CONACYT - Universidad de Sonora, %
        Sonora, %
        Mexico%
    }%
    \corremail{saul.diazinfante@unison.mx}
    %\presentaddress{Present address}
    \runningauthor{F. Baltazar-Larios, F. Delgado-Vences, S. Diaz-Infante}
